SamBaS: Sampling-Based Stochastic Block Partitioning

Community detection is a well-studied problem with applications in domains ranging from networking to bioinformatics. Due to the rapid growth in the volume of real-world data, there is growing interest in accelerating contemporary community detection algorithms. However, the more accurate and statistically robust methods tend to be hard to parallelize. One such method is stochastic block partitioning (SBP) - a community detection algorithm that works well on graphs with complex and heterogeneous community structure. In this paper, we present a sampling-based SBP (SamBaS) for accelerating SBP on sparse graphs. We characterize how various graph parameters affect the speedup and result quality of community detection with SamBaS and quantify the trade-offs therein. To evaluate SamBas on real-world web graphs without known ground-truth communities, we introduce partition quality score (PQS), an evaluation metric that outperforms modularity in terms of correlation with F1 score. Overall, SamBaS achieves speedups of up to 10X while maintaining result quality (and even improving result quality by over 150% on certain graphs, relative to F1 score).

==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix


==> input/authors.tex <==

%%
%% The "author" command and its associated commands are used to define
%% the authors and their affiliations.
%% Of note is the shared affiliation of the first two authors, and the
%% "authornote" and "authornotemark" commands
%% used to denote shared contribution to the research.
\author{Frank Wanye}
% \authornote{Both authors contributed equally to this research.}
\email{wanyef@vt.edu}
\orcid{0000-0002-9154-9132}
\affiliation{%
  \institution{Virginia Tech}
  \streetaddress{620 Drillfield Drive}
  \city{Blacksburg}
  \state{Virginia}
  \postcode{24061-0217}
}

\author{Vitaliy Gleyzer}
\email{vgleyzer@ll.mit.edu}
\affiliation{%
  \institution{MIT Lincoln Laboratory}
  \streetaddress{244 Wood Street}
  \city{Lexington}
  \state{Massachusetts}}

\author{Edward Kao}
\email{edward.kao@ll.mit.edu}
\affiliation{%
  \institution{MIT Lincoln Laboratory}
  \streetaddress{244 Wood Street}
  \city{Lexington}
  \state{Massachusetts}}

\author{Wu-chun Feng}
\email{wfeng@vt.edu}
\affiliation{%
  \institution{Virginia Tech}
  \streetaddress{620 Drillfield Drive}
  \city{Blacksburg}
  \state{Virginia}
  \postcode{24061-0217}
}

%%
%% By default, the full list of authors will be used in the page
%% headers. Often, this list is too long, and will overlap
%% other information printed in the page headers. This command allows
%% the author to define a more concise list
%% of authors' names for this purpose.
% \renewcommand{\shortauthors}{Trovato and Tobin, et al.}

==> input/content-classification.tex <==
%%
%% The code below is generated by the tool at http://dl.acm.org/ccs.cfm.
%% Please copy and paste the code instead of the example below.
%%
% \begin{CCSXML}
% <ccs2012>
%   <concept>
%       <concept_id>10002951.10003227.10003351.10003444</concept_id>
%       <concept_desc>Information systems~Clustering</concept_desc>
%       <concept_significance>300</concept_significance>
%       </concept>
%   <concept>
%       <concept_id>10002950.10003624.10003633.10010917</concept_id>
%       <concept_desc>Mathematics of computing~Graph algorithms</concept_desc>
%       <concept_significance>500</concept_significance>
%       </concept>
%  </ccs2012>
% \end{CCSXML}

% \ccsdesc[300]{Information systems~Clustering}
% \ccsdesc[500]{Mathematics of computing~Graph algorithms}

==> input/graph-generator.tex <==
% %\textbf{WF: This could be better articulated. WF to re-visit.}

% % The 
% To aid in the evaluation of our sampling approach, the graphs we generate need to have the following characteristics:

% \begin{itemize}
%     \item \emph{a known and discernible community structure} to ensure that running community detection on these graphs produces meaningful results, whose quality can be easily measured
%     \item \emph{similarity to real-world graphs} to ensure that our analysis of them is pertinent to real-world data
%     \item \emph{parameters that vary in such a way as to minimize interactions} to ensure that the effects of individual parameters can be isolated and studied
% \end{itemize}

% %a known and discernible community structure to ensure that running community detection on these graphs produces meaningful results, and the quality of these results can be easily measured. They also need to be similar to real-world graphs for our analysis of them to be pertinent to real-world data. And finally, the graph generator needs to have control over various graph parameters in order for them to be individually varied from graph to graph.

% To satisfy these requirements, we generate directed graphs based on the DSCBM~\cite{Karrer2011StochasticNetworks} using the \verb|graph-tool| software library~\cite{Peixoto2014TheLibrary}, 
% %in a similar fashion 
% similar to those generated for the IEEE/Amazon/MIT Streaming Graph Challenge~\cite{Kao2017StreamingPartition}. This ensures that the vertex community memberships are known and that the graph has a well-defined community structure.

% In generating our graphs, we vary the following six parameters $P$:

% \begin{enumerate}
%     \item Number of vertices $|V|$
%     \item Number of communities $C$
%     \item Standard deviation of community sizes $\sigma$
%     \item Strength of community structure $s$, measured by the ratio of the number of edges within communities to the number of edges between communities.
%     \item Strength of high-degree vertices $d^{max}$
%     \item Density $\rho$
% \end{enumerate}

% % \begin{enumerate}
% %     \item \textbf{Number of vertices ($|V|$)}: 
% %     % The number of vertices $|V|$ in the graph is controlled by the size of the community membership array, which is a user-provided parameter to the graph generation function. 
% %     Due to the stochastic nature of the DCSBM-based graph generator, some vertices end up as islands, i.e., zero incoming and outgoing edges. To compensate for this, we generate 113\% of the target number of vertices and then filter out the island vertices.
% %     \item \textbf{Number of communities ($|C|$)}: In this work, we only consider the case of non-overlapping communities $|C|$. Hence, the number of communities is much lower than the number of vertices in the graph.
% %     \item \textbf{Standard deviation of community sizes ($\sigma$)}: The communities in a graph are rarely of the same size. The degree to which the sizes of the communities differ is highly likely to affect the results of community detection, as large communities may absorb smaller ones, or conversely, be broken up into smaller communities. Poor sampling techniques may exacerbate this problem. We control the standard deviation of community sizes $\sigma$ indirectly by sampling the community membership array from a parameterized Dirichlet distribution.
% %     \item \textbf{Strength of community structure ($s$)}: We define the strength of community structure $s$ as the ratio of the number of edges within communities to the number of edges between communities. This parameter is controlled by manually generating the blockmodel from which the graph will be generated. We first generate a blockmodel $B$ such that $B_{i,j} = 1$ if $i == j$, and $\frac{1}{x(|C|-1)}$ otherwise, where $x$ is a user-defined parameter; as $x$ increases, the more the edges are concentrated within communities. In order to ensure the number of edges to and from a community is proportional to its size, we scale $B$ such that $B_{i,j} = B_{i,j} * |C_i| * |C_j|$, where $|C_i|$ and $|C_j|$ are the sizes of the communities $i$ and $j$, respectively.
% %     \item \textbf{Strength of high-degree vertices ($d^{max}$)}: We control the strength of high-degree vertices using a single value, which is the maximum vertex degree $d^{max}$ that can be sampled from the power-law degree distribution without changing the power-law exponent. For the same reasons as above, our control of $d^{max}$ in the generated graph is indirect.
% %     \item \textbf{Density ($\rho$)}: We measure the density $\rho$ of a graph as the total number of edges in a graph, divided by the total number of possible edges in the graph, given by the equation $\rho = \frac{|E|}{|V|(|V|-1)}$ for directed graphs and $\rho = \frac{2|E|}{|V|(|V|-1)}$ for undirected graphs. To vary the density of the generated graphs, we create a graph that is denser than our target parameter, $\rho$, and then delete extraneous edges to meet the desired density. To limit the effect of this deletion on the graph's degree distribution, we select the edges to be deleted uniformly at random.
% % \end{enumerate}

% Note that due to the probabilistic nature of the graph generator, many of these parameters are controlled indirectly, leading to some difference between the expected values of these parameters and the final values in the generated graph.


==> input/old/real-experiments.tex <==
In prior work~\cite{Wanye2019FastSampling}, the above sampling framework was tested on synthetic datasets from the IEEE/Amazon/MIT Streaming Graph Challenge~\cite{Kao2017StreamingPartition}, showing that the quality of $A^S$ is comparable to that of $A$ given a large-enough sample size. In this section, we extend these results to the real-world scenario, and experimentally show that the same result holds for real-world graphs.

% \todo{Why are we doing experiments on real-world graphs?}

\subsection{Real-World Graph Datasets}

\todo{If we get to adding bigger graphs, update this section. Maybe add more dataset parameters to the table? If so, do I add another caption explaining what the parameters are?}

We run our results on 10 web graphs from the Network Data Repository~\cite{Rossi2015TheVisualization}. These graphs are a mixture of directed and undirected graphs that range in size from 326 thousand to 1.9 million vertices, and from 1.5 to 11.7 million edges. Table~\ref{tab:real_graphs} lists the chosen graphs~\footnote{The results presented in Table~\ref{tab:real_graphs} are from examining the graphs using the graph-tool software package, and may differ from the graph descriptions found on http://networkrepository.com/web.php}. While the Network Data Repository does contain larger web graphs, they were excluded due to excessive runtimes.

\todo{Get rid of footnote if smaller graphs aren't added}

\begin{table}
    \caption{Selected real world graphs.}
    \label{tab:real_graphs}
    \begin{tabular}{ccccc}
    \toprule
    ID & Name & Directed? & Number of Vertices $|V|$ & Number of Edges $|E|$ \\
    \midrule
    % R1 & web-polblogs & False & 643 & 2280 \\
    % R2 & web-google & False & 1299 & 2773 \\
    % R3 & web-edu & False & 3031 & 6474 \\
    % R4 & web-EPA & True & 4271 & 8965 \\
    % R5 & web-BerkStan & False & 12305 & 19500 \\
    % R6 & web-webbase-2001 & False & 16062 & 25593 \\
    % R7 & web-indochina-2004 & False & 11358 & 47606 \\
    % R8 & web-spam & False & 4767 & 37375 \\
    % R9 & web-sk-2005 & False & 121422 & 334419 \\
    % R10 & web-frwikinews-user-edits & True & 25042 & 193618 \\
    R1 & web-NotreDame & True & 325729 & 1497134 \\
    R2 & web-arabic-2005 & False & 163598 & 1747269 \\
    R3 & web-Stanford & True & 281903 & 2312497 \\
    R4 & web-italycnr-2000 & True & 325557 & 3216152 \\
    R5 & web-baidu-baike-related & True & 415641 & 3284387 \\
    R6 & web-wikipedia2009 & False & 1864433 & 4507315 \\
    R7 & web-google-dir & True & 875713 & 5105039 \\
    R8 & web-it-2004 & False & 509338 & 7178413 \\
    R9 & web-BerkStan-dir & True & 685230 & 7600595 \\
    R10 & web-uk-2005 & False & 129632 & 11744049 \\
    \bottomrule
    \end{tabular}
\end{table}

\subsection{Experiments}

To evaluate our approach on real-world graphs, we run our sampling framework on each of the graphs in Table~\ref{tab:real_graphs}, using each of the four sampling algorithms described in Section~\ref{sec:sampling_algs}, at various sample sizes ranging from 5\% to 50\% of the vertices in the graph. We use the SBP algorithm (see Section~\ref{sec:sbp}) for the community detection step, and the second, fine-tuning phase of the SBP algorithm for the fine-tuning portion of our sampling framework. Due to the non-deterministic nature of SBP, each combination of graph, sampling algorithm, and sample size is run 15 times, and result aggregation is used for comparison. For our baseline, we run the SBP algorithm sans sampling on the same set of graphs 15 times, and aggregate the results.

These experiments were run on the DragonsTooth cluster at Virginia Tech, using computational nodes with 2 12-core Intel Xeon E5-2680v3 (Haswell) 2.5 GHz processors and 256 GB of 2133 MHz DDR4 memory. We made use of the graph-tool library's~\cite{Peixoto2014TheLibrary} highly optimized parallel implementation of the SBP algorithm, and implemented the sampling algorithms and other parts of the sampling framework using serial python3 code.

\subsection{Quality Metric}\label{sec:quality_metric}

As is often the case with real-world data, our selected real-world graphs are unlabeled, and thus we do not know what the true community members of their vertices are. This prevents us from directly measuring the quality of our results with metrics like accuracy or F1 score. The common approach taken for evaluation community detection on unlabeled graphs is to measure the modularity of the identified community structure. However, higher modularity scores do not always correspond to the optimal community structure~\cite{Fortunato2010CommunityGraphs}.

Given that our chosen algorithm attempts to find the blockmodel that minimizes the minimum description length $H$ of the DCSBM for each graph, adopting $H$ as the measure of quality allows us to determine how well much sampling framework hinders or facilitates inference with the SBP algorithm. In order to allow us to compare $H$ across multiple graphs, we formulate a normalized minimum description length $\tilde{H}$ for each graph,

\begin{equation}\label{eq:h_norm}
    \tilde{H} = 1 - \frac{H - H_{min}}{H_{max} - H_{min}},
\end{equation}

where $H_{max}$ and $H_{min}$ are the maximum and minimum $H$ values for a given graph. We can find a theoretical $H_{max}$ by measuring the value of $H$ if each vertex in a graph is assigned to its own community. This is equal to the minimum description length of the DCSBM at the start of the SBP algorithm. Since we do not know the theoretical value of $H_{min}$ (that is, after all, the entire point of the SBM algorithm), we equate it to the minimum $H$ obtained when running SBP on the graph sans sampling. The $\tilde{H}$ metric is always between the values of $0$ and $1$ (except in the unlikely case that sampling leads to a better $H$ value, in which case $\tilde{H} > 1$), and higher values of $\tilde{H}$ are better, leading to an intuitive metric that can be used for comparison across graphs.

% \todo{What metrics are we collecting?}


==> input/old/real-results.tex <==
In this section, we show and discuss the results of the above experiments.

\subsection{Effect of Sampling Framework on Community Detection Quality}

Figure~\ref{fig:sampling_effectiveness} shows all the $\tilde{H}$ values obtained during the above experiments. While our sampling approach never quite reaches the same values of $\tilde{H}$ as can be obtained without sampling, the results are clearly still very good; every graph has at least some sampling runs with $\tilde{H} > 0.95$. However, it is clear that sampling doesn't work equally well across the different graphs. Graph R9 has a sizeable gap between the $\tilde{H}$ values obtained with and without sampling, while the range of $\tilde{H}$ values obtained with sampling on graph R10 is much larger than on any of the other graphs.

\todo{Make sure I'm doing proper figure descriptions https://www.acm.org/publications/taps/describing-figures/}
 
\begin{figure}[h!]
  \centering
  \includegraphics[width=0.9\linewidth]{input/figures/real/result-distribution-all}
  \caption{The distribution of normalized minimum description lengths $\tilde{H}$ obtained with and without sampling. The horizontal line represents a cut-off value for "good" quality results at $\tilde{H} = 0.95$.}
  \Description{The effectiveness of sampling for community detection.}
  \label{fig:sampling_effectiveness}
\end{figure}

\subsection{Effect of Sampling Algorithm on Community Detection Quality}

Figure~\ref{fig:algs_comparison} shows the maximum $\tilde{H}$ values obtained for each sampling algorithm during the above experiments. From the results, it is clear that typically, the RNN and ES sampling algorithms lead to the best results. However, there is a lot of variability across graphs. RNN sampling performs the best across Graphs R2-R9. In R1, it is second to ES sampling, while in graph 10, it is the worst-performing algorithm, falling below the $\tilde{H} = 0.95$ cut-off.

\begin{figure}[h!]
  \centering
  \includegraphics[width=0.9\linewidth]{input/figures/real/distribution-by-alg2.png}
  \caption{The distribution of normalized minimum description lengths $\tilde{H}$ obtained with four different sampling algorithms at the 30\% sample size for 10 web graphs. The horizontal line represents a cut-off value for "good" quality results at $\tilde{H} = 0.95$.}
  \Description{Boxplots showing the distributions of the normalized description lengths obtained by the Expansion Snowball, Forest Fire, Random Node Neighbor, and Uniform Random algorithms, on 10 web graphs, at the 30 percent sample size. The Random Node Neighbor algorithm is the best performer on all graphs except R1 and R10; on R1 Expansion Snowball outperforms it, while on R10 it is the worst performing algorithm by far. On all but 2 graphs, at least one algorithm has a distribution of normalized description lengths wholly above 0.95.}
  \label{fig:algs_comparison}
\end{figure}


% \begin{figure}[h!]
%   \centering
%   \includegraphics[width=0.9\linewidth]{input/figures/real/comparing-algorithms.png}
%   \caption{The maximum normalized minimum description lengths $\tilde{H}$ obtained with four different sampling algorithms. The horizontal line represents a cut-off value for "good" quality results at $\tilde{H} = 0.95$.}
%   \Description{Comparing the effectiveness of different sampling algorithms.}
%   \label{fig:algs_comparison}
% \end{figure}

\subsection{Effect of Sample Size on Community Detection Quality}

Figure~\ref{fig:sizes_comparison} shows the values of $\tilde{H}$ obtained using the best sampling algorithm for each graph, at sample sizes of 10\%, 30\% and 50\%. As expected, the effectiveness of the sampling framework increases as the sample size increases. However, different graphs require different sample sizes to meet the $\tilde{H} = 0.95$ threshold; R5 meets the threshold even at the sample size of 10\%, while R6 only does so at 50\%. For more detailed results showing all tested sample sizes, see Appendix~\ref{appendix:realgraphs}.

\begin{figure}[h!]
  \centering
  \includegraphics[width=0.9\linewidth]{input/figures/real/comparing-sample-sizes2.png}
  \caption{The distribution of normalized minimum description lengths $\tilde{H}$ obtained by the best performing sampling algorithm for 10 web graphs at samples sizes of 10\%, 30\%, and 50\%. The horizontal line represents a cut-off value for "good" quality results at $\tilde{H} = 0.95$.}
  \Description{Boxplots showing the distributions of the normalized description lengths obtained by the best performing sampling algorithm, on 10 web graphs, at sample sizes of 10, 30, and 50 percent sample size. Only graph R5 shows a distribution of normalized description lengths above 0.95 at the 10 percent sample size. At the 30 percent sample size, the number of graphs with good performance increases to 8, and at the 50 percent sample size, all graphs are showing good performance with sampling.}
  \label{fig:sizes_comparison}
\end{figure}

\subsection{Speedup Obtained via our Sampling Framework}

Figure~\ref{fig:real_speedup} shows the average speedup obtained using our sampling framework at sample sizes of 10\%, 30\% and 50\%. Note that our sampling framework is implemented serially in python3; faster speedups could be obtained by parallelizing the framework and implementing it in a compiled language. Nevertheless, we obtain speedups of up to 33.1X at a sample size of 10\%. At the 30\% sample sizes, which is enough for the majority of graphs to obtain $\tilde{H} > 0.95$, the median speedup is 3.7X. If we further restrict the results to only the best performing algorithm for each graph, the median speedup is 3.3X. Once again, there is a large variability in average speedup across graphs; R10 has much higher average speedups at all sample sizes (going as high as 33.1X), while R1 consistently records some of the lowest average speedups, including a slowdown at 50\% sample size with the ES sampling algorithm. Interestingly, both R1 and R10 have ES sampling as the best-performing sampling algorithm (see Figure~\ref{fig:algs_comparison}), even though their average speedups are on the opposite ends of the spectrum. Despite UR sampling being the simplest of the 4 algorithms, the highest speedups are typically obtained with FF sampling, suggesting that the simplicity of the resulting sample results in longer inference times. RNN sampling, which produced the best $\tilde{H}$ values on 8 out of the 10 graphs, consistently results in lower average speedups.

\begin{figure}[h!]
  \centering
  \includegraphics[width=0.9\linewidth]{input/figures/real/speedup}
  \caption{The average speedup obtained with each of the 4 sampling algorithms at 3 different sample sizes. The horizontal lines show the median speedup at each sample size.}
  \Description{Comparing the speedups for different sampling algorithms and sample sizes.}
  \label{fig:real_speedup}
\end{figure}

% \todo{Are there any other kinds of results we want to show? Sampling algorithms? Sample sizes?}

\subsection{Discussion}

Results on the real-world graphs appear promising. We obtained good results on every dataset, and for most graphs, these results were obtained with a reasonable sample size. Even at the 50\% sample size, all but one algorithm-graph combination results in modest speedups, which could further be improved with a more efficient sample framework implementation.

However, across all the graphs, we encountered a lot of variability in terms of the best sampling algorithm, the sample size sufficient to obtain high quality results, and the speedup obtained for a given sampling algorithm-sample size combination. Thus, it is difficult to recommend a sampling algorithm or sample size for any given graph. As such, the rest of this manuscript describes our experimental approach to explaining this variability.

% \todo{What are the next steps after this discussion?}

==> input/old/synthetic-experiments.tex <==

In this section, we describe a set of experiments for explaining the variability observed in our experiments on real-world graphs. Due to the difficulty in obtaining conclusive results due to the wide range of properties exhibited by real-world graphs, we opt for a graph generator approach. This allows us to produce realistic graphs while having more control over the graph features.

\subsection{Graph Generator}
\todo{Make code available on GitHub under a specific release, add footnote here and in section on sampling framework.}

Our graphs are generated in a similar fashion to those in the IEEE/Amazon/MIT Streaming Graph Challenge~\cite{Kao2017StreamingPartition}. We make use of the graph-tool library~\cite{Peixoto2014TheLibrary} to generate directed graphs based on a DCSBM~\cite{Karrer2011StochasticNetworks} with specified edge probabilities, degree distribution, number of vertices, and vertex-to-community mapping.

First, we generate a vertex-to-community mapping for the desired number of vertices. For this, we draw from a multinomial distribution with probability values for each community drawn from a dirichlet distribution with $\alpha_k = \frac{10}{x}$ for every community $k$, where $x$ is a user-defined community size variation parameter.

\todo{Citation for power law distribution?}

To generate the DSCBM, we first introduce the inter-block edge ratio parameter $s$ such that

\todo{Figure out a better naming for parameters $s$ and $r$, cause this is confusing}

\begin{equation}
    s_{i,j} = \begin{cases}
        \frac{1}{r \cdot (|C| - 1)} & \mbox{if } i = j \\
        1 & \mbox{if } i \not = j,
    \end{cases}
\end{equation} 

where $|C|$ is the number of communities in the graph, and $r$ is a user-defined community strength parameter. We then generate a DCSBM such that $B_{i,j} = s_{i,j} \cdot |C_i| \cdot |C_j|$, where $|C_i|$ and $|C_j|$ correspond to the number of vertices in communities $i$ and $j$, respectively.

Finally, we sample vertex degrees $d_v$ for each vertex $v$ from a discrete power law distribution with a minimum degree of 1, a user-defined maximum vertex degree $d_{max}$, and a user-defined exponent $e$. We set the expected number of edges to $\sum d_v$, and scale our DCSBM such that $\sum B_{i,j} = \sum d_v$. The vertex degrees are randomly split into in-degrees $d_{v,in}$ and out-degrees $d_{v,out}$ with equal probability, such that $d_{v,in} + d_{v,out} = d_v$. This information is then fed into the graph-tool stochastic blockmodel generator to produce a graph that best fits our described blockmodel.

Due to randomness in the graph generation algorithm, as well as the bias towards respecting the parameters of the DCSBM, the resulting graph does not exactly follow the provided degree distribution. However, for the purposes of our experiments, this is acceptable, because the trend in $d_{max}$ and $e$ is consistent with the user-defined parameters (that is, a higher $e$ input by the user leads to a higher $e$ in the generated graph).

We then post-process the graph by deleting randomly selected edges to control the graph sparsity as needed, and then delete all island vertices.

This approach provides us with a high amount of control over a large number of graph parameters, while still producing graphs that are similar to real-world graphs, as will be empirically shown in Section~\ref{sec:comparing_graphs}.

\subsection{Experiments}

In this section, we describe the experiments that we perform, as well as the graph parameters used to generate the synthetic datasets for these experiments. In all, we perform seven experiments, in which we vary the following graph parameters; degree distribution, strength of high-degree vertices, sparsity, strength of community structure, variation in size of communities, the number of communities, and the scale of the graph. In order to accurately attribute the variation in results to the parameters being changed, we strive to only vary one parameter while keeping the remaining 5 as constant as possible.

\todo{Decide if sparsity experiments make sense. Sparsity affects degree distribution, after all. Also, if we do keep this, maybe density is a better word than sparsity.}

Table \ref{tab:exp_metrics} summarizes the metrics we collect about the generated datasets. In addition to the parameters that we set for the graphs, we also collect metrics about their effects on measurable graph parameters. Note that because it is hard to accurately measure the actual power law exponent of the generated graph, we measure the 95th percentile of vertex degrees $d_{95}$ as a proxy for it; the higher the actual power law exponent, the higher the value of $d_{95}$. 

\begin{table}[h!]
    \caption{Metrics Collected and their Notation}
    \label{tab:exp_metrics}
    \begin{tabular}{c|c}
    \toprule
    Metric & Notation \\
    \midrule
    Number of vertices & $|V|$ \\
    Number of edges & $|E|$ \\
    Number of communities & $|C|$ \\
    Community strength & $s$ \\
    Within-to-between community edge ratio & $r$ \\
    Community size variation & $x$ \\
    Standard deviation of community size & $\sigma$ \\
    Maximum vertex degree & $d_{max}$ \\
    Requested power law exponent & $e$ \\
    95th percentile of vertex degrees & $d_{95}$ \\
    \bottomrule
    \end{tabular}
\end{table}

Using synthetic graphs allows us to collect more direct measures of community detection quality like accuracy and F1 score. However, for consistency of results, we evaluate our experiments using the normalized minimum description length $\tilde{H}$ (see Section~\ref{sec:quality_metric}), which we found to be highly correlated with F1 score (see Appendix~\ref{appendix:f1_score_H_correlation}). Finally, similarly to the experiments with real-world graphs, we run combinations of 3 sample sizes (10\%, 30\% and 50\%) using the four sampling algorithms outlined in Section~\ref{sec:sampling_algs} on each graph 10 times to account for natural variability in the algorithm output.

\todo{
\todo{Add Appendix showing correlation of F1 Score and H norm (is that even useful?)}
\todo{Get rid of s, x, and e from the following tables.}
\todo{Decide if we want to use F1 Score - for consistency prolly not}
\todo{Talk about what we expect these parameters to affect, maybe?}
}

\subsubsection{Degree Distribution Experiments}

We vary the degree distribution of the generated graphs by varying the power law exponent $e$ in the range $[-3.5, -1.5]$. Since the number of edges for a graph with a given number of vertices directly depends on the graph's degree distribution, there is no way to prevent $e$ from affecting the sparsity of the graph. Similarly, $e$ is directly related to $d_{max}$, leading to higher $d_{max}$ values as $e$ increases towards 0 (from $d_{max} = 160$ when $e = -3.5$ to $d_{max} = 23K$ when $e = -1.5$). Note that due to the high number of edges at the higher range of $e$ values, we limit the number of vertices in graphs generated for this experiment to keep the runtime reasonable. Table~\ref{tab:dd_graphs} summarizes the parameters of the graphs generated for these experiments.

\begin{table}[h!]
    \caption{Graphs Generated for the Degree Distribution Experiment}
    \label{tab:dd_graphs}
    \begin{tabular}{ccccccccccc}
    \toprule
    ID & $|V|$ & $|E|$ & $|C|$ & $s$ & $r$ & $x$ & $\sigma$ & $d_{max}$ & $e$ & $d_{95}$ \\
    \midrule
    S1 & 95,089 & 134,872 & 336 & 3 & 3.95 & 3 & 194.9 & 160 & -3.5 & 7 \\
    S2 & 95,678 & 153,825 & 336 & 3 & 4.07 & 3 & 207.1 & 355 & -3.0 & 8 \\
    S3 & 97,991 & 213,584 & 336 & 3 & 3.99 & 3 & 195.2 & 1,121 & -2.5 & 11 \\
    S4 & 101,838 & 634,413 & 336 & 3 & 3.82 & 3 & 177.1 & 5,254 & -2.0 & 32 \\
    S5 & 105,225 & 6,486,846 & 336 & 3 & 3.95 & 3 & 190.9 & 22,977 & -1.5 & 393 \\
    \bottomrule
    \end{tabular}
\end{table}

\subsubsection{Strength of High-Degree Vertices Experiments}

We vary the strength of the high-degree vertices by varying $d_{max}$ while keeping every other parameter constant. This does lead to an increase in $|E|$ and $d_{95}$ as $d_{max}$ increases, showing that this parameter has a ``stretching" effect on the graph distribution. Interestingly, the effect of $d_{max}$ on $d_{95}$ appears to be weaker than the effect of $d_{95}$ on $d_{max}$. Table~\ref{tab:supernode_graphs} summarizes the parameters of the resulting graphs.

\begin{table}[h!]
    \caption{Graphs Generated for the Strength of High-Degree Vertices Experiments}
    \label{tab:supernode_graphs}
    \begin{tabular}{ccccccccccc}
    \toprule
    ID & $|V|$ & $|E|$ & $|C|$ & $s$ & $r$ & $x$ & $\sigma$ & $d_{max}$ & $e$ & $d_{95}$ \\
    \midrule
    S6 & 300,591 & 1,002,698 & 582 & 3 & 3.83 & 3 & 311.3 & 596 & -2.1 & 21 \\
    S7 & 299,254 & 1,085,103 & 582 & 3 & 3.97 & 3 & 339.6 & 1,485 & -2.1 & 21 \\
    S8 & 300,709 & 1,262,653 & 582 & 3 & 3.90 & 3 & 326.0 & 4,841 & -2.1 & 23 \\
    S9 & 301,394 & 1,330,587 & 582 & 3 & 3.86 & 3 & 319.7 & 5,634 & -2.1 & 23 \\
    S10 & 302,935 & 1,434,083 & 582 & 3 & 3.87 & 3 & 318.6 & 7,637 & -2.1 & 24 \\
    S11 & 306,094 & 1,629,938 & 582 & 3 & 3.85 & 3 & 313.8 & 14,684 & -2.1 & 26 \\
    \bottomrule
    \end{tabular}
\end{table}

\subsubsection{Sparsity Experiments}

Both $d_{max}$ and $e$ have a strong effect on $|E|$ for roughly the same $|V|$. As such, to find the effect of sparsity on the sampling framework, we combine the results of the two experiments described above.

\subsubsection{Strength of Community Structure Experiments}

We use the within-to-between community edge ratio $r$ as a way to measure the strength of community structure in a graph; the higher this number, the higher the proportion of edges within communities, and the stronger the communities. We indirectly vary $r$ by varying $s$ within the range $[1, 6]$, keeping all other parameters constant. Table~\ref{tab:overlap_graphs} summarizes the parameters of the graphs generated for this experiment.

\begin{table}[h!]
    \caption{Graphs Generated for the Strength of Community Structure Experiments}
    \label{tab:overlap_graphs}
    \begin{tabular}{ccccccccccc}
    \toprule
    ID & $|V|$ & $|E|$ & $|C|$ & $s$ & $r$ & $x$ & $\sigma$ & $d_{max}$ & $e$ & $d_{95}$ \\
    \midrule
    S12 & 306,600 & 1,419,360 & 582 & 1 & 1.32 & 3 & 326.7 & 10,896 & -2.1 & 24 \\
    S13 & 302,745 & 1,425,898 & 582 & 2 & 2.67 & 3 & 340.6 & 10,862 & -2.1 & 24 \\
    S14 & 302,686 & 1,416,219 & 582 & 3 & 3.89 & 3 & 325.4 & 9,120 & -2.1 & 24 \\
    S15 & 302,795 & 1,488,953 & 582 & 4 & 5.13 & 3 & 317.6 & 12,799 & -2.1 & 25 \\
    S16 & 302,140 & 1,480,226 & 582 & 5 & 6.58 & 3 & 336.5 & 13,644 & -2.1 & 25 \\
    S17 & 300,363 & 1,467,761 & 582 & 6 & 7.92 & 3 & 336.8 & 12,780 & -2.1 & 24 \\
    \bottomrule
    \end{tabular}
\end{table}

\subsubsection{Variation in Community Size Experiments}

We vary this by changing the parameter $x$ for the Dirichlet distribution from which the community sizes are drawn within the range $[1, 6]$. Lower values of $x$ lead to more evenly sized communities, and a lower chance that smaller communities get undersampled or merged into larger communities by the SBP algorithm. Table~\ref{tab:variation_graphs} summarizes the resulting graphs for this experiment.

\begin{table}[h!]
    \caption{Graphs Generated for the Variation in Community Size Experiments}
    \label{tab:variation_graphs}
    \begin{tabular}{ccccccccccc}
    \toprule
    ID & $|V|$ & $|E|$ & $|C|$ & $s$ & $r$ & $x$ & $\sigma$ & $d_{max}$ & $e$ & $d_{95}$ \\
    \midrule
    S18 & 308,449 & 1,480,647 & 582 & 3 & 3.27 & 1 & 185.9 & 10,878 & -2.1 & 25\\
    S19 & 304,913 & 1,469,760 & 582 & 3 & 3.63 & 2 & 272.7 & 9,491 & -2.1 & 24\\
    S20 & 303,859 & 1,524,083 & 582 & 3 & 3.85 & 3 & 317.6 & 11,397 & -2.1 & 25\\
    S21 & 302,268 & 1,475,727 & 582 & 3 & 4.15 & 4 & 362.4 & 14,143 & -2.1 & 25\\
    S22 & 300,340 & 1,563,498 & 582 & 3 & 4.49 & 5 & 414.2 & 17,541 & -2.1 & 25\\
    S23 & 300,101 & 1,515,519 & 582 & 3 & 4.58 & 6 & 423.0 & 20,680 & -2.1 & 25\\
    \bottomrule
    \end{tabular}
\end{table}

\subsubsection{Scaling Experiments}

This experiment varies the overall scale of the graph, in terms of both number of edges and vertices, with the aim of identifying how speedup changes as the graph gets larger in size. Because the number of communities tends to grow with the size of the graph, we do not keep $|C|$ constant in this experiment. Table~\ref{tab:scaling_graphs} summarizes the resulting graphs. 

\begin{table}[h!]
    \caption{Graphs Generated for the Scaling Experiments}
    \label{tab:scaling_graphs}
    \begin{tabular}{ccccccccccc}
    \toprule
    ID & $|V|$ & $|E|$ & $|C|$ & $s$ & $r$ & $x$ & $\sigma$ & $d_{max}$ & $e$ & $d_{95}$ \\
    \midrule
    S24 & 64,496 & 273,434 & 268 & 3 & 3.85 & 3 & 149.8 & 3,595 & -2.1 & 23 \\
    S25 & 129,533 & 597,592	& 380 & 3 & 3.90 & 3 & 211.8 & 12,903 & -2.1 & 24\\
    S26 & 259,804 & 1,287,506 & 537 & 3 & 3.84 & 3 & 288.0 & 9,608 & -2.1 & 25\\
    S27 & 522,188 & 2,732,476 & 760 & 3 & 3.85 & 3 & 411.0 & 31,255 & -2.1 & 25\\
    S28 & 1,039,265	& 5,409,988	& 1075 & 3 & 3.87 & 3 & 588.4 & 21,210	& -2.1 & 25\\
    S29 & 2,083,515	& 11,162,085 & 1521 & 3 & 3.87 & 3 & 833.8 & 63,287 & -2.1 & 25\\
    \bottomrule
    \end{tabular}
\end{table}

\subsubsection{Number of Communities Experiments}

In this experiment, we vary the number of communities $|C|$ in the range $[128, 4096]$. By keeping the size of the graph constant, this experiment can also be thought of as measuring the effect of average community size on the quality of sampling results. Interestingly, varying $|C|$ had a significant effect on $d_{max}$ within the generator. We describe the parameters of the graphs generator for this experiment in Table~\ref{tab:num_communities_graphs}.

\begin{table}[h!]
    \caption{Graphs Generated for the Number of Communities Experiments}
    \label{tab:num_communities_graphs}
    \begin{tabular}{ccccccccccc}
    \toprule
    ID & $|V|$ & $|E|$ & $|C|$ & $s$ & $r$ & $x$ & $\sigma$ & $d_{max}$ & $e$ & $d_{95}$ \\
    \midrule
    S30 & 301,090 & 1,481,756 & 128 & 3 & 3.91 & 3 & 1493.3 & 25,109 & -2.1 & 22 \\
    S31 & 302,724 & 1,449,717 & 256 & 3 & 3.75 & 3 & 681.2 & 18,684 & -2.1 & 24 \\
    S32 & 302,645 & 1,509,053 & 512 & 3 & 3.89 & 3 & 368.4 & 16,860 & -2.1 & 25 \\
    S33 & 304,063 & 1,471,727 & 1,024 & 3 & 3.94 & 3 & 188.9 & 9,472 & -2.1 & 26 \\
    S34 & 307,653 & 1,495,872 & 2,048 & 3 & 3.92 & 3 & 93.0 & 6,403 & -2.1 & 27 \\
    S35 & 309,301 & 1,453,166 & 4,096 & 3 & 3.94 & 3 & 46.6 & 3,188 & -2.1 & 28 \\
    \bottomrule
    \end{tabular}
\end{table}

% \todo{Combines tables into 1 large table? Move to Appendix? Add a row for standard deviation for the "constant" parameters?}

% \begin{table}[h!]
%     \caption{Large Table Test}
%     \label{tab:test}
%     \begin{tabular}{ccccccccccc|ccccccccccc}
%     \toprule
%     \multicolumn{11}{c|}{Degree Distribution Experiment} & 
%     \multicolumn{11}{c}{Strength of High-Degree Vertices Experiment} \\
%     ID & $|V|$ & $|E|$ & $|C|$ & $s$ & $r$ & $x$ & $\sigma$ & $d_{max}$ & $e$ & $d_{95}$ &
%     ID & $|V|$ & $|E|$ & $|C|$ & $s$ & $r$ & $x$ & $\sigma$ & $d_{max}$ & $e$ & $d_{95}$ \\
%     \midrule
%     S25 & \\
%     S26 & \\
%     S27 & \\
%     S28 & \\
%     S29 & \\
%     S30 & \\
%     \toprule
%     \multicolumn{11}{c|}{Strength of Community Structure Experiment} & 
%     \multicolumn{11}{c}{Variation in Community Size Experiment} \\
%     ID & $|V|$ & $|E|$ & $|C|$ & $s$ & $r$ & $x$ & $\sigma$ & $d_{max}$ & $e$ & $d_{95}$ &
%     ID & $|V|$ & $|E|$ & $|C|$ & $s$ & $r$ & $x$ & $\sigma$ & $d_{max}$ & $e$ & $d_{95}$ \\
%     \midrule
%     S25 & \\
%     S26 & \\
%     S27 & \\
%     S28 & \\
%     S29 & \\
%     S30 & \\    
%     \toprule
%     \multicolumn{11}{c|}{Scaling Experiment} &
%     \multicolumn{11}{c}{Number of Communities Experiment} \\
%     ID & $|V|$ & $|E|$ & $|C|$ & $s$ & $r$ & $x$ & $\sigma$ & $d_{max}$ & $e$ & $d_{95}$ &
%     ID & $|V|$ & $|E|$ & $|C|$ & $s$ & $r$ & $x$ & $\sigma$ & $d_{max}$ & $e$ & $d_{95}$ \\
%     \midrule
%     S25 & \\
%     S26 & \\
%     S27 & \\
%     S28 & \\
%     S29 & \\
%     S30 & \\
%     \bottomrule
%     \end{tabular}
% \end{table}

% \begin{enumerate}
%     \item \textbf{Sparsity}: The sparsity of the graph refers to its edge density, i.e. the ratio of total number of edges in the graph to the total number of possible edges in the graph. \hl{How does this affect sampling?} Simply adding or subtracting edges from the graph post-generation could significantly affect the vertex degree distribution, as well as the within-to-between community edge ratio. To minimize the affect of sparsity on both these parameters, we control sparsity by adding a constant value to the minimum and maximum vertex degrees, thus translating the degree distribution along the x-axis without affecting its shape. The generated graphs are summarized in Table~\ref{tab:sparsity_graphs} in Appendix \ref{appendix:syngraphs}.

%     \item \textbf{Degree distribution}: The shape of the degree distribution affects how many vertices of a particular degree exist in the graph. \hl{How does this affect sampling?} To vary this parameter, we vary the exponent $e$ of the truncated power law degree distribution, such that $-3.5 \leq e \leq 3.5$, ensuring that we take into account degree distributions that favor both low-degree and high-degree vertices. It should be noted that for a fixed graph size, the degree distribution has a direct effect on the sparsity of the graph, and thus the interaction between these two parameters could affect our results. The generated graphs are summarized in Table~\ref{tab:deg_distribution_graphs} in Appendix \ref{appendix:syngraphs}.

%     \item \textbf{Community size}: The size of the community refers to the number of vertices that belong to it. Intuitively, larger communities would lead to a better performance by our sampling framework, since it's more likely that the sampling algorithm includes many vertices from each community. Thus, we would like to ascertain how small the communities can get before the effectiveness of our framework deteriorates. To vary the community size, we keep the graph size constant, and vary the number of communities present in the graph. The generated graphs are summarized in Table~\ref{tab:community_size_graphs} in Appendix \ref{appendix:syngraphs}.

%     \item \textbf{Community overlap}: This controls the strength of the community structure within the graph. A high within-to-between community edge ratio $r$ means that the communities are well-defined, whereas a ratio of $1$ would indicate that there is no community structure in the graph. Intuitively, the less well-defined the communities, the higher the sample size needed to capture the community structure of the graph. We vary this parameter such that $1.0 \leq r \leq 6.0$. Due to the stochastic nature of the graph generator, the value of $r$ in the generated graphs varies slightly from our setting. The generated graphs are summarized in Table~\ref{tab:edge_ratio_graphs} in Appendix \ref{appendix:syngraphs}.
    
%     \todo{Is overlap confusing because of overlapping community detection?}

%     \item \textbf{Variation in community size}: This refers to the relative difference in sizes of the communities. When some communities are much smaller than others, community detection algorithms find it hard to detect the smaller communities~\cite{}. This could be further compounded by sampling, since these communities become even smaller. The community sizes in our graph generator are drawn from a Dirichlet distribution with $k$ parameters, such that each parameter $p = \frac{10}{x}$, where $k$ is the number of communities in the graph, $x$ is the variation in community size. The higher the value of $x$, the more varied the community sizes in the generated graph. We vary $x$ such that $1.0 \leq x \leq 6.0$. The generated graphs are summarized in Table~\ref{tab:community_size_var_graphs} in Appendix \ref{appendix:syngraphs}.

%     \item \textbf{Supernode connectivity}: This is represented by the vertex degree of the high-degree vertices in the graph. \hl{Such vertices can be though of as `hubs,' and the number of connections they have can have a significant effect on graph traversal.} To control this parameter, we vary the maximum vertex degree in the graph while keeping the minimum vertex degree constant. It should be noted that this does skew the vertex degree distribution and has an effect on graph sparsity, and their interactions could affect our results. The generated graphs are summarized in Table~\ref{tab:connectivity_graphs} in Appendix \ref{appendix:syngraphs}.

%     \item \textbf{Scaling}: This refers to the total number of vertices in the graph. Due to the super-linear runtime of many community detection algorithms, our sampling framework should provide a super-linear speedup for a given sample size, as the graph size increases. Additionally, the speedup should increase in an exponential fashion as the sample size decreases. \hl{Finally, since the number of communities tends to scale sublinearly to the graph size, it is likely that as the graph size increases, the sample size needed to achieve good results decreases}. To test these assumptions, we generate two sets of graphs graphs varying in size $s$, such that $1000 \leq s \leq 1024000$. For one set of graphs, we set the number of communities $c = s^{0.35}$ to mimic sublinear scaling of the number of communities. For the other set, we set $c = s * 0.5^8$. This helps keep the number of block merge iterations of the stochastic block partitioning algorithm to a relatively constant value, and thus helps ensure that the size of the graph is the main driving force between any speedups obtained. The generated graphs are summarized in Table~\ref{tab:size_graphs} in Appendix \ref{appendix:syngraphs}.
% \end{enumerate}

\subsection{Similarity to Real-World Graphs}\label{sec:comparing_graphs}

To show that results on our synthetic graphs are comparable to results on real-world graphs, we compare our graphs to the smallest 25 web graphs from the Network Data Repository~\cite{Rossi2015TheVisualization}. Because we do not know the true community structure of these web graphs, we cannot measure $|C|$, $r$ or $\sigma$ for the real-world graphs. Additionally, since many of the graph features depend on and scale with other features, most of comparisons are performed using ratios. As can be seen in Figure~\ref{fig:graph_comparison}, our synthetically generated graphs are comparable to real-world graphs based on the following: 

\begin{itemize}
    \item Ratio of number of edges $|E|$ to number of vertices $|V|$
    \item Ratio of maximum vertex degree $d_{max}$ to number of vertices $|V|$
    \item Ratio of average vertex degree $d_{avg}$ to maximum vertex degree $d_{max}$
    \item Relative size of largest connected component (as defined by $\frac{|V^C|}{|V|}$, where $|V^C|$ is the number of vertices in the largest connected component
    \item Ratio of 95th percentile of vertex degrees $d_{95}$ to number of vertices $|V|$
    \item Clustering coefficient
\end{itemize}

\begin{figure}[h!]
  \centering
  \includegraphics[width=0.9\linewidth]{input/figures/comparison/Graph Comparison.png}
  \caption{Comparing various features of real-world web graphs to our synthetically generated graphs.}
  \Description{A figure showing comparisons between our synthetically generated graphs and the real-world graphs in terms of 6 parameters.}
  \label{fig:graph_comparison}
\end{figure}


==> input/old/synthetic-results.tex <==
In this section, we describe the results we have obtained on the experiments outlined in the previous section. We summarize the results obtained in order to answer the following questions: 
% For each experiment, we attempt to answer the following questions: 

\begin{itemize}
    \item How do the graph parameters affect the quality of results with sampling?
    \item How do the graph parameters affect the sampling conditions necessary for high quality results?
    \item How do the graph parameters affects the speedup of sampling?
\end{itemize}

\subsection{Effect on Quality of Results with Sampling}

Here, we discuss how the degree distribution, strength of high-degree vertices, strength of community structure, variation in community size, the scale of the graph, and the number of communities affects the quality of results, in terms of $\tilde{H}$, that can be achieved with sampling. Similarly to the real-world experiments, we consider a good result to be one where $\tilde{H} \geq 0.95$.

First, we look at parameters that have to do with deal with the communities themselves. Generally, we find that as the strength of community structure increases (Figure~\ref{fig:syn_quality_structure}), and the number of communities decreases (Figure~\ref{fig:syn_quality_communities}), the sampling approach performs better. These results are intuitive; stronger and larger communities mean that it's more likely for sampling to effectively capture most of the community structure within a graph. However, we also find that the sampling approach performs better as the standard deviation in community size increases (see Figure~\ref{fig:syn_quality_variation}). This is unintuive in that one would expect more variation in community size to lead to smaller communities being undersampled, which would in turn lead to the community detection algorithm not discovering them. While we do see this decrease in the number of communities being discovered (Figure~\ref{fig:syn_communities_variation}), this seems to lead to stronger communities being formed overall, leading to a decrease in $H$.

\todo{How do we explain the community size variation results better? Is this a problem with the generated graph, the metric, or the algorithm? Does this suggest that there IS a resolution limit for community detection with SBP?}

Next, we look at the remaining 3 parameters. We find that as the degree distribution becomes less steep (and the graph becomes less sparse), the $\tilde{H}$ values get closer to $1.0$ (see Figure~\ref{fig:syn_quality_dd}). A similar trend, albeit much less pronounced, is observed with an increase in the strength of high-degree vertices (see Figure~\ref{fig:syn_quality_supernode}). This is expected, since higher connectivity means it's a) easier to traverse the graph, and b) less likely that a sample contains small disconnected components.

\subsection{Effect on Sampling Conditions Necessary for High Quality results}

Here, we discuss how the six parameters varied in our experiments affect a) which sampling algorithms lead to higher $\tilde{H}$ values, and b) how small a sample size is needed to achieve high quality results.

\subsection{Effect on Speedup with Sampling}

Here, we discuss the effect of the six parameters on the speedup obtained using our sampling framework. For brevity, we present results only from the sampling algorithm that is found to have the highest mean $\tilde{H}$ at a sample size of 30\% for each graph.

% \begin{itemize}
%     \item How has the final quality of community detection with sampling been affected?
%     \item How has the best-performing sampling algorithm been affected?
%     \item How has the sample size needed to achieve an acceptable quality of community detection been affected?
%     \item How has the speedup been affected?
% \end{itemize}

% Note that for the sake of brevity, we only show results where the experiment does have an effect on these 4 questions.

% \subsection{Experiments with Sparsity}

% \todo{F1 Score, Communities obtained? Size of preserved communities? Sample size needed? Best algorithm?}

% \subsection{Experiments with Degree Distribution}

% \todo{F1 Score, Communities obtained? Size of preserved communities? Sample size needed? Best algorithm?}

% \subsection{Experiments with Strength of Community Structure}

% \todo{F1 Score, Communities obtained? Size of preserved communities? Sample size needed? Best algorithm?}

% \begin{figure}[h!]
%   \centering
%   \includegraphics[width=0.9\linewidth]{input/figures/synthetic/overlap-effectiveness.png}
%   \caption{Comparing the effect of strength of community structure on the effectivess of the sampling framework (left), and on the best-performing sampling algorithm (right).}
%   \Description{TODO.}
%   \label{fig:overlap_results}
% \end{figure}

% \subsection{Experiments with Community Size Variation}

% \todo{F1 Score, Communities obtained? Size of preserved communities? Sample size needed? Best algorithm?}

% \subsection{Experiments with Supernode Strength}

% \todo{F1 Score, Communities obtained? Size of preserved communities? Sample size needed? Best algorithm?}

% \subsection{Experiments with Scaling}

% \todo{F1 Score, Communities obtained? Size of preserved communities? Sample size needed? Best algorithm?}

% \subsection{Experiments with Number of Communities}

% \todo{F1 Score, Communities obtained? Size of preserved communities? Sample size needed? Best algorithm?}

% \begin{figure}[h!]
%   \centering
%   \includegraphics[width=0.9\linewidth]{input/figures/synthetic/communitysize-effectiveness.png}
%   \caption{Comparing the effect of the number of communities on the effectiveness of the individual sampling algorithms (left), and on the speedup obtained with the sampling approach (right).}
%   \Description{TODO.}
%   \label{fig:communitysize_results}
% \end{figure}

\subsection{Discussion}

\todo{Discuss the results. Why? How? What do they mean?}


==> input/threshold_sampling.tex <==

Previous work has shown that sampling can 
%not only 
preserve community structure
%, but also 
as well as allow for the structure to be inferred for unsampled vertices~\cite{Wanye2019FastSampling,Maiya2010SamplingStructure}. However, the graphs used in those efforts are much denser than the graphs we target in this manuscript.
% The median web graphs that we run our sampling approach on have a median density of 0.00002 (number of edges present divided by maximum possible number of edges), an order of magnitude lower than the lowest density of the graphs in either of the previous works.
These differences naturally suggest that the sampling strategies that perform best on web graphs %would 
differ from the more dense graphs in previous work because low-density graphs present a unique challenge for sampling. Lower graph densities imply that the degree distribution of the graph is skewed towards the low 
%degree 
end. As such, it is much more likely to lead to vertices with low degrees being selected in the sample. This presents a problem because the community-related information content of an edge is proportional to the vertex degrees of the two vertices connected by said edge~\cite{Kao2019HybridInteractions}. If the sampled subgraph contains more low-degree vertices, then the total information content of the edges in this subgraph will be comparatively low. Island vertices would provide absolutely no useful information.

To counteract this effect, we propose a simple thresholding scheme, where vertices are only considered for a sample if their vertex degree is above a threshold $t$. This ensures that only higher-degree vertices are included in the sample and increases the chances that a vertex has multiple edges in the sample itself, thereby increasing its information content.

